OpenAsp: A Benchmark for Multi-document Open Aspect-based Summarization

The performance of automatic summarization models has improved dramatically in recent years. Yet, there is still a gap in meeting specific information needs of users in real-world scenarios, particularly when a targeted summary is sought, such as in the useful aspect-based summarization setting targeted in this paper. Previous datasets and studies for this setting have predominantly concentrated on a limited set of pre-defined aspects, focused solely on single document inputs, or relied on synthetic data. To advance research on more realistic scenarios, we introduce OpenAsp, a benchmark for multi-document \textit{open} aspect-based summarization. This benchmark is created using a novel and cost-effective annotation protocol, by which an open aspect dataset is derived from existing generic multi-document summarization datasets. We analyze the properties of OpenAsp showcasing its high-quality content. Further, we show that the realistic open-aspect setting realized in OpenAsp poses a challenge for current state-of-the-art summarization models, as well as for large language models.

==> 01Introduction.tex <==
\subsection{Introduction-Old}


When faced with a large body of text, a summary is an effective means to get a concise version of the salient content. At times, the text-consumer has some prior background knowledge or informational goal, and fancies a focused summary around a specific matter. This real-world necessity is addressed by tasks such as aspect-based summarization \citep[ABS;][]{angelidis2018summarizing} \shmulik{TODO: fix oposum} and query-focused summarization \citep[QFS;][]{daume2006qfs}.
%, where the output summary is biased around an input request.

An aspect is traditionally a concise predefined phrase that is broadly related to the topic or domain of the source text(s) \cite{angelidis2018summarizing}\shmulik{TODO: fix oposum}. Such generic pre-specified requests allow for a high-level partition of information in the source text. For example, it may be sufficient to summarize an article about a natural disaster around ``recovery'' or ``geography'' \citep{ahuja2022aspectnews}.
%\os{cite such a dataset} \cite{meng-etal-2021-facetsum}.
Most ABS benchmarks follow this ``closed-set'' definition of an aspect (see \autoref{tab:related-datasets}).

Alternatively, a query is inherently fluid, allowing great variance in length, specificity and format \citep{carmel2006query}. A query can range from a single word \citep{baumel-etal-2014-query}, to a question \cite{wang2022squality}, and even a broad multi-sentence request \citep{dang2005overview}.

A question such as ``What facilities were damaged
in the Oaxacan region?'' 
%A question such as ``what was the extent of damage in the event?''
essentially assumes the reader is already proficient in the content of the text \citep{ahuja2022aspectnews}. Meanwhile, overly broad requests tend to render standard generic summaries \citep{Baumel_Cohen_Elhadad_2016}.


An \textit{open}-aspect is the middle ground between a standard aspect and a query. The natural flow of seeking information assumes the reader is not yet aware of the text, but likely has some prior knowledge about what to look for, such as a sub-topic within the specific text. 
Few datasets have applied this construct by using wikipedia articles with relevant concepts \cite{tan2020summarizing} 
or sub-titles \cite{yang2022oasum} serving as the aspects. These datasets rely on a single source document per instance. We view the multi-document setting, as an additional appealing factor to consider for real-world scenarios, such as in search results.

Collecting datasets for tasks like ABS and QFS poses a challenging undertaking that includes reading large input texts and writing out the focused summaries.
%\shmulik{maybe add that its hard to find them in the wild, like generic summarization, and to build them its hard. (but maybe its too much for here).}
This is especially true in the multi-document setting which consists of even more text, and requires consolidation of information from across documents. For these reasons, most relevant datasets are collected synthetically, with lower-quality input documents, aspects and expected output summaries. Few datasets \citep{angelidis2018summarizing, angelidis2021extractive, ahuja2022aspectnews} are an exception to this, however their summaries only center around a handful of aspects.
See \autoref{tab:related-datasets} for a comparison of related datasets.

We introduce, \openasp{}\shmulik{OS - TODO we need to add placeholder for link or footnote stating we'll release \openasp{} to public}, the first multi-document open-aspect-based summarization dataset, collected manually to render high-quality summaries for varying aspects. We devise an efficient protocol that overcomes the burdening task of manually preparing summaries for large document sets. Namely, the aspect-based summaries are derived from generic reference summaries of prominent multi-document summarization (MDS) datasets (DUC; \citeauthor{nist2002DUCWebsite}, \citeyear{nist2002DUCWebsite} and MultiNews; \citeauthor{fabbri-etal-2019-multi}, \citeyear{fabbri-etal-2019-multi}). See \autoref{fig:annotation_ui_main} for an example of open-aspect-based summaries extracted from a generic summary. The dataset contains 1,310 aspect-based summaries, split to train, validation and test sets, enabling methodological modeling for the task. We implement and analyze several baseline models that demonstrate the challenging nature of the task and dataset, even for recent high-performance large language models.






% A query is inherently fluid in terms of its format and goal, allowing great variance in length, specificity of . It can  allowing, e.g., long generic descriptions \os{cite DUC 2006}, questions \os{cite long-form QA}, or highly specific requests \os{cite something relevant}. Alternatively, an aspect is traditionally a short predefined phrase that is broadly related to the topic or domain of the source text(s) \os{cite a paper that defines this kind of aspect}.

% To facilitate research on the ABS task, several datasets have been developed. Most datasets approach the task in the single-document setting, \shmulik{no need the i.e. part IMHO.}i.e., the input includes just one document to summarize around a given aspect \os{cite these datasets}. Some practical scenarios call for a multi-document setting\shmulik{OS - you want to cite MDS here?}, where a reader is confronted with many related texts. The one dataset \os{cite multidoc ABS} that does address the multi-document setup is compiled synthetically from \os{how is it compiled, and why is this not ideal?}\shmulik{automatically derive using heuristics (on wikipedia pages \& sections)}. Collecting summaries manually from large bodies of text, and multi-document sets particularly, is a challenging feat. Only few ABS datasets \os{cite manually collected ABS datasets} were collected manually by \shmulik{crowdsourced} experts and \os{anything to say about them?} \shmulik{small and tackle specific, predefined set of aspects.}
% %Moreover, the datasets are predominantly compiled synthetically from Wikipedia \os{cite} or \os{some other domain (cite)}, apart from \os{non synthetic ds} that targets \os{what does it target?}. 

% While predefined domain-level aspects (e.g., \os{examples of such sets and their domain}) can be sufficient to allow a high level partition of information, a need for a more fine-grained focus may arise for each specific text or reader. The reader may wish to simply request a subtopic within the text, which is essentially a blend of an aspect and a query. \os{citet OA with open-aspects} is a dataset for single-document open ABS, that was prepared by automatically scraping Wikipedia articles, with subtitles serving as open aspects\shmulik{there is also AnyAspect \citet{tan2020summarizing}}. \os{what is a possible problem in OAsum?}\shmulik{its highly synthetic, and its not MDS.}

% We introduce, \openasp{}, the first multi-document open-aspect-based summarization dataset, collected manually to render high-quality summaries for varying aspects (\os{see table... comparing ABS and manual multi-doc QFS datasets...}). We devise an efficient protocol to overcome the burdening task of manually preparing summaries for large document sets. Namely, the aspect-based summaries are derived from generic reference summaries of prominent multi-document summarization (MDS) datasets \os{DUC and MultiNews citations} (see \os{figure 1} for an example of opn-aspect-based summaries extracted from a generic summary). The dataset contains \os{how many aspect-based summaries?} split to train, validation and test sets, enabling methodological modeling for the task. We implement and analyze several baseline models that demonstrate the challenging nature of the task and dataset, even for recent high-performance large language models.



% % Today, humanity is facing an explosion of data which often hinders one from traversing all available information. Therefore various methods have been proposed to automatically summarise documents while preserving the most salient information \citep{gambhir2017recent, yoshida2014dependency, goldstein2000multi, zhang2016extractive, chen2019sentence, yang2014enhancing, see2017get, ailem2019topic}.  

% The vast majority of summarization literature focuses on the generic summarization task, which aims to produce a comprehensive summary of a topic, covering a range of possible points of interest based solely on the content of the input document(s) \citep{gambhir2017recent, gong2001generic}. 

% However, in realistic scenarios, people often need a summary focused on a specific aspect of the topic. For example, given documents about a new COVID drug, medical practitioners may be interested in the drug's side-effects, whereas patients may be more concerned about usage instructions. In this context, \emph{side-effects} and \emph{instructions} represent different aspects of the COVID drug topic, and users may require separate summaries pertaining to each.

% We noted that there is no formal definition of "aspect" in the summarization field, and its interpretation varies across different works. In this work, we consider an aspect of a topic, in light of a set of documents on the topic, to be a sub-topic contained in the documents and for which a complete and meaningful summary can be derived from the documents.

% The \emph{Aspect-based Summarization} task \citep{hayashi2021wikiasp, amplayo2021aspect, frermann2019inducing, tan2020summarizing, meng2021bringing, angelidis2021extractive, ahuja2022aspectnews} aims to provide a targeted summary of one document or more from a specific aspect.
% % the aspect-based summarization task outputs a focused summary dealing with a specific aspect of the information.

% The main challenge of developing aspect-based summarization systems is the lack of large annotated datasets comprised of documents paired with multiple aspect-based summaries. To address this challenge, existing works tend to focus on specific domains and aspects as well as synthetic datasets. These works are considered to have "closed-aspect" approaches since they predefine a closed aspect list and do not respond well to new aspects introduced post-training. 

% While predefined aspect lists may suffice in some domains, such as product or service reviews where users are typically interested in recurring aspects, in other domains, particularly in the news domain, aspects of different topics can be highly diverse, prompting users to request summaries for various aspects.
 
% % \liat{add a paragraph: while being limited to a few aspects in the product reviews domain might be enough, in the news domain is totally different story}

% Few recent works \citep{tan2020summarizing, ahuja2022aspectnews} do aim to support any aspect request, and thereby are considered to have an open-aspect approach. However, similar to earlier works, they lack annotated datasets that cover multiple domains and aspects for evaluation purposes. 

% Furthermore, it is worth noting that most existing works on aspect-based summarization in the news domain are primarily focused on summarizing single-document inputs. However, in order to summarize the large amounts of news articles that often have on each topic, there is a need for a system that can deal with a set of documents as input. 

% % creating a system which will be able to summarize more than a single document the Multi-document input 
% % \liat{to give the motivation to multi-document in the news domain}
% % However, the more challenging scenario lies in handling multi-document inputs, as the process of creating an annotated dataset becomes significantly more demanding and time-consuming. 

% \liat{to add works on multi-document in the news domain and emphasis their problems}

% Our work has the following contributions: 
% \begin{itemize}
% \item Creating a quality and diversified dataset with gold standard summaries of diverse aspects. This dataset can be used as a first benchmark for the multi-document aspect-based summarization task in the open aspect approach.
% \item Presenting a cost-effective annotation protocol for creating quality aspect-based summarization benchmarks by utilizing manually annotated generic summarization datasets.
% \item Analyzing the abilities of baseline models in addressing the task, where the input is multiple documents on a common topic and an aspect phrase, and the model output an abstractive summary related to this aspect.
% \end{itemize}

% In Section....


% % Task and its motivation, and what was addressed so far

% % * Generic motivation for ABS: Real-world scenarios call for summaries focused on a specific aspect of interest. ABS aims to provide targeted summaries of one document (or more) from multiple perspectives.
% %         - Check ABS papers for their motivation
        
% % * In some cases, it is sufficient to have pre-specified lists of aspects, regardless of the source(s), as in product/service reviews. Most existing benchmarks addressed the task in such a manner.

% % * Moreover, ABS benchmarks usually address the task for single-doc inputs, and are prepared as synthetic datasets.

% % * However, in the general case, the task is 
% %         - open aspect - exemplify/illustrate, 
% %         - needed also for the highly useful multidoc setting - exemplify use cases (show in figure)

% % * This setting was addressed only through synthetic data generation, not manually  





==> Figures/dataset_lengths_cumsum.tex <==
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/lengths_main_density_docs_only.png}    %{images/lengths_main_density_docs_only_4k.svg}
    % \includegraphics[width=\linewidth]{images/lengths_main.png}
    \caption{The distribution of document-sets token-lengths in \openasp{}. The \textcolor{red}{red} line in the left graph marks summaries with up to 128 words (80.5\% of the dataset). In the right figure, the \textcolor{orange}{orange}, \textcolor{red}{red} and {\color{asparagus}green} lines mark popular model maximum input sizes of document sets with up to 1024, 4096 and 16384 words (3.5\%, 32.2\% and 88.2\% of the data respectively).}
    %\os{what's the 1e-5 at the top?}\shmulik{thats the scale, so it 1e-5*8. its very tiny and including all 5 zeros is noisy. i can try do something like 2e-5, 4e-5, 6e-5... if you think its better}}
    %\openasp{}'s probability distribution of word-lengths for summaries (left) and document sets (right). The \textcolor{red}{red} line in the left graph marks summaries with up to 128 words (80.46\% of the dataset). In the right figure, the \textcolor{orange}{orange}, \textcolor{red}{red} and {\color{asparagus}green} lines mark the document sets with up to 1024, 4096 and 16384 words (3.51\%, 32.21\% and 88.24\% of the data respectively).}
    \label{fig:data-lengths}
\end{figure}

==> Figures/human_evaluation_results_fig.tex <==
\begin{figure}[t]
% \centering
\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{images/aspect-relevancy_fig.png}  
    \caption{}
    \label{SUBFIGURE LABEL 1}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=.95\linewidth]{images/reference-relevancy_fig.png}  
    \caption{}
    \label{SUBFIGURE LABEL 2}
\end{subfigure}
\caption{The scores distribution for the 'Aspect-relevancy' (a) and 'Reference-relevancy' (b) measures is presented. A total of 20 aspect-based summaries produced by fine-tuned BART were evaluated.}
\label{fig:human_evaluation}
\end{figure}

==> Tables/curation_phase_examples.tex <==
\begin{table}[t]
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|cccc}

\toprule
Guid & Aspect Label & Original Aspect Label & Summary & Original Summary \midrule
bucket-list adventure/U495/mnews-valid.209436.A & bucket-list adventure & Nicole takes Chester on bucket-list adventure & But despite his health problems, Elliott is helping him get the most out of his last days. "I slept on it, and woke up knowing it was the right thing to do," she tells WTVM. Chester, likely 13 or 14, now has a Facebook page and is checking off a "bucket list" to ensure he has an "awesome final ride," Elliott tells the New York Daily News. So far, Chester has had a spa day with a milk and oatmeal bath and a shopping spree for new toys. There have also been plenty of treats, like "a famous Nathans hot dog" and a sundae. "I am taking it a day at a time and trying to give him normal doggy experiences that he may have never had the chance to do before, and a ton of spoiling," says Elliott. Next on the list: dinner at a restaurant, a day at the beach, a boat ride, and a birthday party with other rescued animals. & aaa
\bottomrule
\end{tabular}%}
\caption{The size of the \openasp{} dataset splits. ``\# Topics'' denotes the number of document sets, ``\# Instances'' is the total number of aspect-based summaries, and ``\# Docs'' is the total number of source documents.}
\label{tab:curation_phase_examples}
\end{table}

==> Tables/figure1.tex <==
\begin{table}[h]
\resizebox{\linewidth}{!}{%

\begin{tabular}{|ll|}
\hline
 &                                                                                                                                                                                                                                                       \\
 & {\ul \textbf{Generic Summary:}}                                                                                                                                                                                                                       \\
 &                                                                                                                                                                                                                                                       \\
 & Antarctica is larger than China and India combined.                                                                                                                                                                                                   \\
 & Ninety-eight percent of the continent is under ice.                                                                                                                                                                                                   \\
 & It is drier than the Sahara desert.                                                                                                                                                                                                                   \\
 & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Antarctica has been important on three fronts--geopolitical, \\ future economic development and scientific research.\end{tabular}}                                                                         \\
 &                                                                                                                                                                                                                                                       \\
 & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}In 1959 an international treaty placed a hold on the territorial\\ claims of seven nations, placed Antarctica off-limits for \\ military bases and opened it for scientific research to all.\end{tabular}} \\
 &                                                                                                                                                                                                                                                       \\
 &                                                                                                                                                                                                                                                       \\
 & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Currently sixteen nations oversee sixty-eight research \\ bases there.\end{tabular}}                                                                                                                       \\
 &                                                                                                                                                                                                                                                       \\
 & \multicolumn{1}{c|}{\textbf{...}}                                                                                                                                                                                                                     \\
 & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Antarctica is believed to hold unknown quantities of \\ strategic metals and billions of gallons of oil.\end{tabular}}                                                                                     \\
 &                                                                                                                                                                                                                                                       \\
 & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}The United States and Great Britain grudgingly accepted\\ the pact changes.\end{tabular}}                                                                                                                  \\
 &                                                                                                                                                                                                                                                       \\
 & \multicolumn{1}{c|}{\textbf{...}}                                                                                                                                                                                                                     \\
 & \multicolumn{1}{c|}{\textbf{}}                                                                                                                                                                                                                        \\ \hline
\end{tabular}


}
    \caption{\liat{change to figure 1 instead table}A generic summary from DUC on the topic \textbf{\textit{Antarctica}} with the marked sentences for each of the 4 identified aspect labels: 
    \textcolor{overview}{\textit{Overview of Antarctica}}, \textcolor{research}{\textit{Research in Antarctica}}, \textcolor{importance}{\textit{Antarctica's importance}}, and \textcolor{territ}{\textit{Territorial claims}}.}
    \label{fig:annotation_ui_main}
\end{table}


% \begin{table}[h]
% \resizebox{\linewidth}{!}{%


% \begin{tabular}{|ll|}
% \hline
%  &                                                                                                                                                                                                                                                       \\
%  & {\textbf{Generic Summary:}}                                                                                                                                                                                                                       \\
%  &                                                                                                                                                                                                                                                       \\
%  &  \setulcolor {overview} 
%  \ul{Antarctica is larger than China and India combined.}                                                                                                                                                                                                   \\
%  &                                                                                                                                                                                                                                                       \\
%  & \setulcolor {overview} 
%  \ul{Ninety-eight percent of the continent is under ice.}                                                                                                                                                                                                   \\
%  &                                                                                                                                                                                                                                                       \\
%  & \setulcolor {overview} 
%  \ul{It is drier than the Sahara desert.}                                                                                                                                                                                                                   \\
%  &                                                                                                                                                                                                                                                       \\
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {importance} 
%  \ul{Antarctica has been important on three fronts--geopolitical,} \\ \setulcolor {importance} 
%  \ul{future economic development and scientific research.}\end{tabular}}                                                                         \\
%  &                                                                                                                                                                                                                                                       \\
%  &                                                                                                                                                                                                                                                       \\
%  & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {territ} 
%  \ul{In 1959 an international treaty placed a hold on the territorial}\\ \setulcolor {territ} 
%  \ul{claims of seven nations, placed Antarctica off-limits for} \\ \setulcolor {territ} 
%  \ul{military bases and opened it for scientific research to all.}\end{tabular}} \\
%  &                                                                                                                                                                                                                                                       \\
%  &                                                                                                                                                                                                                                                       \\
%  &                                                                                                                                                                                                                                                       \\
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {research} 
%  \ul{Currently sixteen nations oversee sixty-eight research} \\ \setulcolor {research} 
%  \ul{bases there.}\end{tabular}}                                                                                                                       \\
%  &                                                                                                                                                                                                                                                       \\
%  & \multicolumn{1}{c|}{\textbf{...}}                                                                                                                                                                                                                     \\
%  &                                                                                                                                                                                                                                                       \\
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {importance} 
%  \ul{Antarctica is believed to hold unknown quantities of} \\ \setulcolor {importance} 
%  \ul{strategic metals and billions of gallons of oil.}\end{tabular}}                                                                                     \\
%  &                                                                                                                                                                                                                                                       \\
%  &                                                                                                                                                                                                                                                       \\
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {territ} 
%  \ul{The United States and Great Britain grudgingly accepted}\\ \setulcolor {territ} 
%  \ul{the pact changes.}\end{tabular}}                                                                                                                  \\
%  &                                                                                                                                                                                                                                                       \\
%  & \multicolumn{1}{c|}{\textbf{...}}                                                                                                                                                                                                                     \\
%  & \multicolumn{1}{c|}{\textbf{}}                                                                                                                                                                                                                        \\ \hline
% \end{tabular}

% }
%     \caption{\liat{change to figure 1 instead table}A generic summary from DUC on the topic \textbf{\textit{Antarctica}} with the marked sentences for each of the 4 identified aspect labels: 
%     \textcolor{overview}{\textit{Overview of Antarctica}}, \textcolor{research}{\textit{Research in Antarctica}}, \textcolor{importance}{\textit{Antarctica's importance}}, and \textcolor{territ}{\textit{Territorial claims}}.}
%     \label{fig:annotation_ui_main}
% \end{table}



% \begin{table}[h]
% \resizebox{\linewidth}{!}{%

% \begin{tabular}{|lll|}
% \hline
%  &                                                                                                                                                                                                                                                           &                                \\
%  & \textbf{Generic Summary:}                                                                                                                                                                                                                                 & {\ul \textbf{}}                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & Antarctica is larger than China and India combined.                                                                                                                                                                                                       &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & Ninety-eight percent of the continent is under ice.                                                                                                                                                                                                       &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & It is drier than the Sahara desert.                                                                                                                                                                                                                       &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Antarctica has been important on three \\ fronts--geopolitical, future economic \\ development and scientific research.\end{tabular}}                                                                          &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}In 1959 an international treaty placed a hold on the \\ territorial claims of seven nations, placed Antarctica \\ off-limits for military bases and opened it for \\ scientific research to all.\end{tabular}} &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Currently sixteen nations oversee sixty-eight\\ research bases there.\end{tabular}}                                                                                                                            &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & \multicolumn{1}{c}{\textbf{...}}                                                                                                                                                                                                                          & \multicolumn{1}{c|}{\textbf{}} \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Antarctica is believed to hold unknown quantities \\ of strategic metals and billions of gallons of oil.\end{tabular}}                                                                                         &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  &                                                                                                                                                                                                                                                           &                                \\
%  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}The United States and Great Britain grudgingly \\ accepted the pact changes.\end{tabular}}                                                                                                                     &                                \\
%  &                                                                                                                                                                                                                                                           & \multicolumn{1}{c|}{\textbf{}} \\
%  & \multicolumn{1}{c}{\textbf{...}}                                                                                                                                                                                                                          &                                \\
%  & \multicolumn{1}{c}{\textbf{}}                                                                                                                                                                                                                             & \multicolumn{1}{c|}{\textbf{}} \\ \hline
% \end{tabular}

% }
%     \caption{A generic summary on the topic \textbf{\textit{Antarctica}} with the marked sentences for each of the 4 identified aspect labels: 
%     \textcolor{deepskyblue}{\textit{Overview of Antarctica}}, \textcolor{darkpastelgreen}{\textit{Research in Antarctica}}, \textcolor{deeppink}{\textit{Antarctica's importance}}, and \textcolor{darkorange}{\textit{Territorial claims}}.}
%     \label{fig:annotation_ui_main}
% \end{table}







% \begin{table}[h]
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|lcll|}
% \hline
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & \multicolumn{2}{l}{{\textbf{Generic Summary:}}}                                                                                                                                                                                                                          & {\ul \textbf{}}                \\
%  &                      &                                                                                                                                                                                                                                                       &                                \\
%  & 1.                   & \setulcolor {deepskyblue}
% \ul{Antarctica is larger than China and India combined.}                                                                                                                                                                                                   &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & 2.                   & \setulcolor {deepskyblue}
% \ul{Ninety-eight percent of the continent is under ice.}                                                                                                                                                                                                   &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & 3.                   & \setulcolor {deepskyblue}
% \ul{It is drier than the Sahara desert.}                                                                                                                                                                                                                   &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & 4.                   & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {deeppink}
% \ul{Antarctica has been important on three fronts--geopolitical}, \\ \setulcolor {deeppink}
% \ul{future economic development and scientific research}.\end{tabular}}                                                                         &                                \\
%  &                      &                                                                                                                                                                                                                                                       &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & 5.                   & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {darkorange}
% \ul{In 1959 an international treaty placed a hold on the territorial}\\ \setulcolor {darkorange}
% \ul{claims of seven nations, placed Antarctica off-limits for} \\ \setulcolor {darkorange}
% \ul{military bases and opened it for scientific research to all.}\end{tabular}} &                                \\
%  &                      &                                                                                                                                                                                                                                                       &                                \\
%  &                      &                                                                                                                                                                                                                                                       &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & 6.                   & \setulcolor {darkpastelgreen}
% \ul{Currently sixteen nations oversee sixty-eight research bases there.}                                                                                                                                                                                   &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  &                      & \multicolumn{1}{c}{\textbf{...}}                                                                                                                                                                                                                      & \multicolumn{1}{c|}{\textbf{}} \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & 8.                   & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {deeppink}
% \ul{Antarctica is believed to hold unknown quantities of} \\ \setulcolor {deeppink}
% \ul{strategic metals and billions of gallons of oil.}\end{tabular}}                                                                                     &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       &                                \\
%  & 9.                   & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\setulcolor {darkorange}
% \ul{The United States and Great Britain grudgingly accepted the} \\ \setulcolor {darkorange}
% \ul{pact changes.}\end{tabular}}                                                                                                                 &                                \\
%  & \multicolumn{1}{l}{} &                                                                                                                                                                                                                                                       & \multicolumn{1}{c|}{\textbf{}} \\
%  & \multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{...}}                                                                                                                                                                                                                      &                                \\
%  &                      & \multicolumn{1}{c}{\textbf{}}                                                                                                                                                                                                                         & \multicolumn{1}{c|}{\textbf{}} \\ \hline
% \end{tabular}
% }
%     \caption{A generic summary on the topic \textbf{\textit{Antarctica}} with the marked sentences for each of the 4 identified aspect labels: 
%     \textcolor{deepskyblue}{\textit{Overview of Antarctica}}, \textcolor{darkpastelgreen}{\textit{Research in Antarctica}}, \textcolor{deeppink}{\textit{Antarctica's importance}}, and \textcolor{darkorange}{\textit{Territorial claims}}.}
%     \label{fig:annotation_ui_main}
% \end{table}

% \begin{table}[h]
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{ll}
% \multicolumn{2}{l}{{\ul \textbf{Generic Summary:}}}                                                                                                                                                                                                                             \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{1.} & \colorbox{LightCyan}{Antarctica is larger than China and India combined.}                                                                                                                                                                                                    \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{2.} & \colorbox{LightCyan}{Ninety-eight percent of the continent is under ice.}                                                                                                                                                                                                    \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{3.} & \colorbox{LightCyan}{It is drier than the Sahara desert.}                                                                                                                                                                                                                    \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{4.} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\colorbox{pastelpink}{Antarctica has been important on three fronts--geopolitical,} \\ \colorbox{pastelpink}{future economic development and scientific research.}\end{tabular}}                                                                          \\
%                        &                                                                                                                                                                                                                                                        \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{5.} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\colorbox{teagreen}{In 1959 an international treaty placed a hold on the territorial} \\ \colorbox{teagreen}{claims of seven nations, placed Antarctica off-limits for military} \\ \colorbox{teagreen}{bases and opened it for scientific research to all.}\end{tabular}} \\
%                        &                                                                                                                                                                                                                                                        \\
%                        &                                                                                                                                                                                                                                                        \\
%                        &                                                                                                                                                                                                                                                        \\
% 6.                     & \colorbox{lemonchiffon}{Currently sixteen nations oversee sixty-eight research bases there.}                                                                                                                                                                                    \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{}   & \multicolumn{1}{c}{\textbf{...}}                                                                                                                                                                                                                       \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{8.} & \begin{tabular}[c]{@{}l@{}}\colorbox{pastelpink}{Antarctica is believed to hold unknown quantities of strategic}\\ \colorbox{pastelpink}{metals and billions of gallons of oil.}\end{tabular}                                                                                                        \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{9.} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\colorbox{teagreen}{The United States and Great Britain grudgingly accepted the} \\ \colorbox{teagreen}{pact changes.}\end{tabular}}                                                                                                                  \\
%                        &                                                                                                                                                                                                                                                        \\
%                        &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{c}{}   & \multicolumn{1}{c}{\textbf{...}}                                                                                                                                                                                                                      
% \end{tabular}
% }
%     \caption{A generic summary on the topic \textit{Antarctica} with the marked sentences for each of the 4 identified aspect labels: 
%     \colorbox{LightCyan}{\textit{Overview of Antarctica}}, \colorbox{lemonchiffon}{\textit{Research in Antarctica}}, \colorbox{pastelpink}{\textit{Antarctica's importance}}, and \colorbox{teagreen}{\textit{Territorial claims}}.}
%     \label{fig:annotation_ui_main}
% \end{table}




% \setulcolor {blue}
% \ul{\textit{Overview of Antarctica}}


% \begin{table}[h]
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{cl}
% \multicolumn{2}{l}{{\ul \textbf{Generic Summary:}}}                                                                                                                                                                                                                             \\
% \multicolumn{1}{l}{}   &                                                                                                                                                                                                                                                        \\
% 1.                     & \colorbox{LightCyan}{Antarctica is larger than China and India combined.}                                                                                                                                                                                                    \\
% 2.                     & \colorbox{LightCyan}{Ninety-eight percent of the continent is under ice.}                                                                                                                                                                                                    \\
% 3.                     & \colorbox{LightCyan}{It is drier than the Sahara desert.}                                                                                                                                                                                                                    \\
% 4.                     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}\colorbox{pastelpink}{Antarctica has been important on three fronts--geopolitical,} \\ \colorbox{pastelpink}{future economic development and scientific research.}\end{tabular}}                                                                          \\
% \multicolumn{1}{l}{}   &                                                                                                                                                                                                                                                        \\
% 5.                     & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}\colorbox{teagreen}{In 1959 an international treaty placed a hold on the territorial} \\ \colorbox{teagreen}{claims of seven nations, placed Antarctica off-limits for military} \\ \colorbox{teagreen}{bases and opened it for scientific research to all.}\end{tabular}} \\
% \multicolumn{1}{l}{}   &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{l}{}   &                                                                                                                                                                                                                                                        \\
% \multicolumn{1}{l}{6.} & \colorbox{lemonchiffon}{Currently sixteen nations oversee sixty-eight research bases there.}                                                                                                                                                                                   \\
%                        & \multicolumn{1}{c}{\textbf{...}}                                                                                                                                                                                                                       \\
% 8.                     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Antarctica is believed to hold unknown quantities of strategic\\ metals and billions of gallons of oil.\end{tabular}}                                                                                       \\
% \multicolumn{1}{l}{}   &                                                                                                                                                                                                                                                        \\
% 9.                     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}The United States and Great Britain grudgingly accepted the \\ pact changes.\end{tabular}}                                                                                                                  \\
% \multicolumn{1}{l}{}   &                                                                                                                                                                                                                                                        \\
%                        & \multicolumn{1}{c}{\textbf{...}}                                                                                                                                                                                                                      
% \end{tabular}
% }
%     \caption{A generic summary on the topic \textit{Hurricane Gilbert} with 3 aspect labels and the respective aspect-based summaries, on our annotation interface.}
%     \label{fig:annotation_ui_main}
% \end{table}

==> Tables/most_common_aspect_labels.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ll}
\textbf{Aspect Label} & \textbf{Topic Titles}                                                                                                               \\ \hline
government response   & \begin{tabular}[c]{@{}l@{}}United States drought\\ Floods in China\\ Flooding in Ohio\\ Tropical Storm Harvey in Texas\end{tabular} \\ \hline
criticism             & \begin{tabular}[c]{@{}l@{}}Amnesty International\\ US Organic Foods Market\\ Judge Robert Bork\end{tabular}                         \\ \hline
personal life         & \begin{tabular}[c]{@{}l@{}}Erich Honecker obituary\\ Lucille Ball\\ Alan Greenspan\end{tabular}                                     \\ \hline
popularity            & \begin{tabular}[c]{@{}l@{}}The 'Seinfeld' series\\ US Organic Foods Market\\ Debate on term limits\end{tabular}                     \\ \hline
family response       & \begin{tabular}[c]{@{}l@{}}Kennedy Plane Crash\\ Terry Anderson's abduction\end{tabular}                                           
\end{tabular}%
}
\caption{}
\label{tab:most-common-aspect-labels}
\end{table}
